Lepton Flavour Violating tau and mu decays induced by scalar leptoquark

We show that the scalar leptoquark Yukawa couplings generate a significant lepton flavour violation. We compute the light scalar leptoquark contributions to the branching ratios (Br) of the lepton flavour violating (LFV) decays $\ell \to \ell_i \ell_j \bar{\ell}_j$ and $\ell \rightarrow \ell^{\prime} \gamma$ with (i,j = e,$\mu$). We discuss the role of the relevant input parameters to these decay rates which are the Yukawa couplings ($h_{a\ell}$) with ($a=u,c,t$), the light scalar mass $M_{S_{1}}$ and the mixing angle $\sin2\theta_{LQ}$. We investigate the experimental limits from $(g-2)_\mu$, $\mu-e$ conversion and $\pi \to e \nu_e, \mu \nu_\mu$ to get constraint on the input parameter space. We predict that the upper limits on the branching ratios of $\tau \to \ell_i \ell_j \bar{\ell}_j $ can reach the experimental current limits. We also show that it is possible to accommodate both $\tau \to \ell_i \ell_j \bar{\ell}_j$ and $\tau \to \ell\gamma$ branching ratios for certain choices of LQ parameters.

==> box_LQ.tex <==
\unitlength=1bp%

\begin{feynartspicture}(432,504)(4,5.3)
%=======================================================
\FADiagram{}
\FAProp(0.,10.)(10.,10.)(0.,){/Straight}{1}
%\FALabel(18.5,4.5)[t]{$(a)$}
\FALabel(5.,8.5)[t]{$\ell$}
%\FAProp(36.,10.)(26.5,10.)(0.,){/Straight}{-1}
%\FALabel(33.8,7.1)[br]{$\ell_i$}
%\FAProp(18.5,16.6)(18.5,26.5)(0.,){/Sine}{0}
%\FALabel(15.5,20.)[bl]{$V$}
%\FAProp(10.,10.)(26.5,10.)(0.,){/ScalarDash }{1}
%\FAProp(10.,10.)(18.5,16.6)(-0.4,){/Straight }{1}
%\FAProp(18.6,16.6)(26.5,10.)(-0.4,){/Straight }{1}
%\FAProp(18.5,26.5)(28.5,31.5)(0.,){/Straight }{1}
%\FALabel(30.,26.5)[t]{$\ell_j$}
%\FAProp(18.5,26.5)(28.5,24.5)(0.,){/Straight }{-1}
%\FALabel(30.,33.5)[t]{$\ell_j$}
%\FALabel(12.,16.02)[b]{$u^c_a$}
%\FALabel(24.6,16.02)[b]{$u^c_a$}
%\FALabel(18.5,7)[b]{$S_k$}
%\FAVert(10.,10.){0}
%\FAVert(26.5,10.){0}
%\FAVert(18.5,16.6){0}
%\FAVert(18.5,26.5){0}
%====================================================
%\FADiagram{}
%\FAProp(30.,10.)(40.,10.)(0.,){/Straight}{1}
%\FALabel(48.5,4.5)[t]{$(b)$}
%\FALabel(35.,8.5)[t]{$\ell$}
%\FAProp(56.,10.)(66.5,10.)(0.,){/Straight}{1}
%\FALabel(63.8,7.1)[br]{$\ell_i$}
%\FAProp(30.,10.)(66.5,10.)(0.,){/Straight }{1}
%\FAProp(40.,10.)(48.,16.6)(-0.4,){/ScalarDash}{1}
%\FAProp(48.,16.6)(56.5,10.)(-0.4,){/ScalarDash}{1}
%\FAProp(48.,16.6)(48.,26.5)(0.,){/Sine}{0}
%\FAProp(48.,26.6)(58.,24.)(0.,){/Straight }{-1}
%\FAProp(48.,26.6)(58.,31.)(0.,){/Straight }{1}
%\FALabel(45.5,20.)[bl]{$V$}
%\FALabel(54.5,16.02)[b]{$S_k$}
%\FALabel(42.5,16.02)[b]{$S_k$}
%\FALabel(48.5,7)[b]{$u^c_a$}
%\FALabel(58.,23.5)[t]{$\ell_j$}
%\FALabel(58.,30.)[t]{$\ell_j$}
%\FAVert(40.,10.){0}
%\FAVert(56.2,10.){0}
%\FAVert(48.,16.6){0}
%\FAVert(48.,26.5){0}
%===================================================
\end{feynartspicture}


